Towards a Better Understanding of VR Sickness: Physical Symptom Prediction for VR Contents

We address the black-box issue of VR sickness assessment (VRSA) by evaluating the level of physical symptoms of VR sickness. For the VR contents inducing the similar VR sickness level, the physical symptoms can vary depending on the characteristics of the contents. Most of existing VRSA methods focused on assessing the overall VR sickness score. To make better understanding of VR sickness, it is required to predict and provide the level of major symptoms of VR sickness rather than overall degree of VR sickness. In this paper, we predict the degrees of main physical symptoms affecting the overall degree of VR sickness, which are disorientation, nausea, and oculomotor. In addition, we introduce a new large-scale dataset for VRSA including 360 videos with various frame rates, physiological signals, and subjective scores. On VRSA benchmark and our newly collected dataset, our approach shows a potential to not only achieve the highest correlation with subjective scores, but also to better understand which symptoms are the main causes of VR sickness.

==> sections/ack.tex <==
This work was supported by Institute for Information $\&$ communications Technology Promotion(IITP) grant funded by the Korea government(MSIT) (No.2017-0-00780, Development of VR sickness reduction technique for enhanced sensitivity broadcasting).

==> sections/sec_5_3.tex <==
To understand the prediction performance of the proposed VRSA framework, we observed the expected frame generated by the trained deep neural store network. Figure 9 shows the visual results predicted by the proposed deep neural store network for Video 1 (simple motion) and Video 9 (complex motion) on \cite{41}. In Fig. 9 (a) and (b), the first and second rows indicate the original NFOV frames and the expected NFOV frames by the trained neural store network. The last row indicates the prediction error (i.e., difference, $\textbf{d}_{t}$). As shown in the Fig. 9(a), Video 1 with the simple motion pattern was predicted well. On the other hand, in Fig. 9(b), the deep neural store network trained with normal videos with non-exceptional motion could not well predict Video 9 because this video has exceptional velocity and rapid rotation. As shown in the third row of Fig. 9(b), it can be seen that most of the prediction error occur around the rapidly varying area such as acceleration and rapid rotation in Video 9. This result indicates that deep neural store network trained by videos with non-exceptional motion could detect the specific region causing excessive VR sickness.

Figure 10 shows the visual results predicted by the proposed deep neural store network for Video 3 (static on the boat) and Video 15 (normal driving). As shown in the Fig. 10(a), Video 3 with even 10 fps was predicted well because the original videos did not have any motion and complex textures. Actually, the total SSQ score for Video 3 is range of [3, 7] according to the frame rate (total SSQ for Video3 with 10 fps: 6.96 and total SSQ for Video3 with 60 fps: 3.48). It means that visual information of VR content has an influence on the VR sickness. Fig. 10(b) shows the visual results for Video 15. The total SSQ scores for Video 15 with 30 fps and 60 fps were 34.8 and 33.06, respectively. That is, original video 15 with high frame rate could not lead to severe VR sickness. On the other hand, total SSQ score for Video 15 with 10 fps was 64.38. As shown in Fig. 10(b), the prediction error between the original frames and the expected frames by the trained deep neural store network is much higher than other results. This result indicates that the level of VR sickness for the same video can vary with frame rate. By the proposed deep neural store network can detect the specific region at each frame, which is related to severe VR sickness. Through the deep comparison and sickness score prediction networks, the level of VR sickness can be predicted reliably.

